Bringing the SciBar Detector to the Booster Neutrino Beam

This document presents the physics case for bringing SciBar, the fully active, finely segmented tracking detector at KEK, to the FNAL Booster Neutrino Beam (BNB) line. This unique opportunity arose with the termination of K2K beam operations in 2005. The physics that can be done with SciBar/BNB can be put into three categories, each involving several measurements. First are neutrino cross section measurements which are interesting in their own right, including analyses of multi-particle final states, with unprecedented statistics. Second are measurements of processes that represent the signal and primary background channels for the upcoming T2K experiment. Third are measurements which improve existing or planned MiniBooNE analyses and the understanding of the BNB, both in neutrino and antineutrino mode. SciBar and BNB have both been built and operated with great success. As a result, the cost of SciBar/BNB is far less than building a detector from scratch and both systems are well understood with existing detailed and calibrated Monte Carlo simulations. The performance expectations assumed in this document are therefore well-grounded in reality and carry little risk of not meeting expectations.

==> sections/goals.tex <==
\chapter{Physics Goals}
\label{chap:goals}

%\begin{sideways}
\begin{tabular}{|c|c|c|c|c|c|c|} \hline
%\multicolumn{4}{|c|}{Physics Case}\\\hline
   \multirow{2}{*}{Class}  
&  \multirow{2}{*}{Measurement}  
&  Loc. 1  &  Loc. 2 & Loc. 3 & Loc. 4 & MB alone\\
&  &  \$$x$k  & \$$x\prime$k & \$$x\prime\prime$k & \$$x\prime\prime\prime$k & \$$0$k \\\hline
\multirow{4}{*}{Help T2K}
& $\numu$ CCQE         & A & B & A & B & x \\\cline{2-7}
& $\numu$ NC$\pi^0$    & C & D & C & D & x \\\cline{2-7}
& $\numubar$ CCQE      & E & F & E & F & x \\\cline{2-7}
& $\numubar$ NC$\pi^0$ & G & H & G & H & x \\\cline{1-7}
\multirow{3}{*}{Leverage MB} 
& $\nubar$ in $\nu$ mode  & I & J & A & B & x \\\cline{2-7}
& Intrinsic $\nue$        & K & L & C & D & x \\\cline{2-7}
& $\numu$ Disappearence   & M & N & E & F & x \\\cline{1-7}
\multirow{3}{*}{Scibar Physics} 
& Multi-track Recon & O & P & A & B & x \\\cline{2-7}
& CCQE                    & Q & R & C & D & x \\\cline{2-7}
& Coherent $\pi$          & S & T & E & F & x \\\cline{1-7}
\end{tabular}
%\end{sideways}

\section{How to Define Physics Goals}
\label{sec:def}

\subsection{Balancing Cost, Flux, and Energy Spectrum}
\label{subsec:balance}

\section{Oscillation Measurements}
\label{sec:osc}

\section{Cross Section Measurements}
\label{sec:xsec}

\section{Diagnostic Measurements}
\label{sec:diag}

\subsection{$\pi$ and K Fluxes}
\label{subsec:pi-k}

\subsection{$\nu$ and  $\nubar$ Fluxes}
\label{subsec:nu-nubar}

\subsection{Intrinsic $\nue$  Contamination}
\label{subsec:nue}




